Regret Bound Balancing and Elimination for Model Selection in Bandits and RL

We propose a simple model selection approach for algorithms in stochastic bandit and reinforcement learning problems. As opposed to prior work that (implicitly) assumes knowledge of the optimal regret, we only require that each base algorithm comes with a candidate regret bound that may or may not hold during all rounds. In each round, our approach plays a base algorithm to keep the candidate regret bounds of all remaining base algorithms balanced, and eliminates algorithms that violate their candidate bound. We prove that the total regret of this approach is bounded by the best valid candidate regret bound times a multiplicative factor. This factor is reasonably small in several applications, including linear bandits and MDPs with nested function classes, linear bandits with unknown misspecification, and LinUCB applied to linear bandits with different confidence parameters. We further show that, under a suitable gap-assumption, this factor only scales with the number of base algorithms and not their complexity when the number of rounds is large enough. Finally, unlike recent efforts in model selection for linear stochastic bandits, our approach is versatile enough to also cover cases where the context information is generated by an adversarial environment, rather than a stochastic one.

==> experiments.tex <==


\section{Experiments}
number of features $d = 10$,
number of actions $A = 100$,
$7$ instances of LinUCB as base learners,
fixed action set, Gaussian noise on rewards with different variances: 
    \url{http://flatboard/p/XHaQ6mj1_Zw}
\section{Limitations: Different dependence on $n$}

What if the different base algorithms satisfy regret guarantees with a different exponent on $n$. 
See Jamboard for an example where we cannot retain the optimal $T$ exponent in the worst case.




==> optimization.tex <==




\section{Convex optimization}

We may be able to use these techniques to devise adaptive procedures to select the optimal learning rate. Throughout this section we assume the objective is to optimize a (convex) function $f: \mathbb{R}^d \rightarrow \mathbb{R}$. We study two settings. First the case where the learner has access to possibly noisy function evaluations and gradients, and second the case where the learner has access to only (possibly noisy) gradient evaluations. We provide results for both the noiseless and the noisy cases. 



Let $f$ be $L-$ smooth:

\begin{equation*}
    \| \nabla f(x) - \nabla f(y) \|_2 \leq L \| x-y\|_2
\end{equation*}

And convex:

\begin{equation}
    f(x) + \langle \nabla f(x), y-x \rangle \leq f(y) 
\end{equation}

and:

\begin{equation}
    f(y) \leq f(x) + \langle \nabla f(x) , y-x \rangle + \frac{L}{2} \| y-x \|^2
\end{equation}

Recall the following theorem:

\begin{theorem}
Let $f: \mathbb{R}^d \rightarrow \mathbb{R}$ be a $L-$Lipschitz convex function and $x^* = \arg\min_x f(x)$. then Gradient Descent with step-size $\eta \leq \frac{1}{L}$ satisfies the following:

\begin{equation}\label{equation::conv_opt_guarantee}
    f(x_k) \leq f(x^*)  + \frac{\| x_0 -x^* \|^2 }{2\eta k}
\end{equation}

In particular $\frac{L \| x_0 - x^* \|^2 }{\epsilon}$ iterations suffice to find an $\epsilon-$approximate optimal value $x$ (for $\eta = 1/L$). 
\end{theorem}

Equation \ref{equation::conv_opt_guarantee} implies, if the GD algorithm is ran with an estimator $\hat{L}$ for $L$ (in other words setting $\eta = \frac{1}{\hat{L}}$) with iterates $\{ x_k^{(\hat{L})}\}$ and $\hat{L} \leq L$:

\begin{equation}\label{equation::inst_regret}
    f(x^{(\hat{L})}_k) \leq f(x^* ) + \frac{\hat{L} \| x_0  - x^* \|^2}{2k}
\end{equation}
Let $r^{(\hat{L})}_t = f(x^{(\hat{L})}_k) - f(x^*)$, Equation \ref{equation::inst_regret} implies a bound $r_k^{(\hat{L})} \leq \frac{ \hat{L} \| x_0 - x^* \|^2 }{ 2k }$.

Let's assume a \textbf{known} upper bound $\| x_0 - x^* \| \leq B$. 

We define the cumulative regret of a an algorithm with learning rate $\hat{L}$ as:

\begin{equation}
    \mathcal{R}(T, \hat{L})= \sum_{k=1}^T r_t^{(\hat{L})}
\end{equation}

By assumption, whenever $\hat{L} \leq L$: 

\begin{equation*}
    \mathcal{R}(T, \hat{L}) \leq \frac{\hat{L}B}{2}\sum_{k=1}^T \frac{1}{k} \leq \hat{L}B\log(T).
\end{equation*}

Let's assume we have access to a Lipschitz constant upper bound $L_M$ that is guaranteed to satisfy: $L_M > L^*$. We can always compute a Lipschitz constant lower bound $L_0$ by picking two points $x', x''$ in the domain $\{ x \text{ s.t. }\|x - x_0\| \leq B \}$ and defining $L_0 = \frac{\| \nabla f(x') - \nabla f(x'') \| }{\| x' - x'' \|}$. 

Recall that in case $\hat{L} << L$, GD with learning rate $\eta = \frac{1}{\hat{L}}$ may yield a linear regret. 

The same approach as in the general section should work. 



\subsection{Stochastic Gradient Descent}

The setup in \cite{rakhlin2011making} may prove useful.

We also make use of the results in \cite{harvey2019tight}.  


\subsection{Noise and Strong Convexity}

The following Lemma borrowed from \cite{rakhlin2011making} holds:

\begin{lemma}[Lemma 2]
Let $\delta \in (0, 1/e)$ and $T \geq 4$. Suppose $F$ is $\tau-$strongly convex over a convex set $\mathcal{W}$, and that the gradients satisfy $\| \hat{\mathbf{g}}_t\|^2 \leq G^2$ with probability $1$. Then if we pick $\eta_t = c/\rho t$ for some constant $c> 1/2$, such that $2c$ is a whole number, it hodls with probability at least $1-\delta$ that for any $t \in [4c^2 +4c, \cdots, T-1, T]$ that:
\begin{equation*}
    \| w_t - w^* \|^2\leq \frac{12c^2 G^2}{\rho^2 t} + 8(12G+1)G\frac{c \log(\log(t)/\delta )}{\rho t}
\end{equation*}
Where $w_t$ corresponds to the $t-$th iterate of projected stochastic gradient descent with step sizes $\eta_t$. 
\end{lemma}

We work under the assumption the learner has access to lower and upper bounds on $F$ strong convexity parameter $\tau_{\min} \leq \tau_* \leq \tau_{\max}$ and lower and upper bounds on its smoothness parameter $\mu_{\min} \leq \mu_*  \leq \mu_{\max}$. We assume knowledge of $G$, although this assumption can be obviated. 

Let $\{\tau_i\}_{i=1}^M$ and $\{\mu_ i\}_{i=1}^M$ be a (logarithmic) grid of parameters. And let:

\begin{equation*}
    \mathcal{M} = \{ (\tau, \mu) | \tau \in \{ \tau_i\}_{i=1}^M, \mu \in \{ \mu_i \}_{i=1}^M \text{ and } \tau_i \leq \mu_i \}.
\end{equation*}

We 

We propose the following algorithm:






\begin{algorithm}
    $\Ical_1 \gets [M]$\tcp*{set of active learners}
\For{round $t=1, 2, 3, \dots$}{
    Pick the base learner as
    $i_t \in \argmin_{i \in \Ical_t} \wt \Rcal_i(n_{i}(t-1) + 1)$\;
    
    Play learner $i_t$ and receive reward $r_t$\;
    
    $\mathcal I_{t+1} \gets \mathcal I_{t}$\;
    
    \ForEach{learner $i \in \mathcal I_t$}{
    \If{$\frac{U_i(t)}{n_i(t)} + c\sqrt{\frac{\ln (n_i(t) / \delta)}{n_i(t)}}
    + \frac{\wt \Rcal_i(n_i(t))}{n_i(t)} < \max_{j \in \Ical_t} \frac{U_j(t)}{n_j(t)} - c\sqrt{\frac{\ln (n_j(t) / \delta)}{n_j(t)}}$}{
    $\Ical_{t+1} \gets \Ical_{t+1} \setminus \{ i \}$\tcp*{remove misspecified learner}
    }
    }
}
\caption{General Regret Balancing and Elimination Algorithm}
\label{alg:balanced_elim_strong_convexity}
\end{algorithm}










